Heterogeneous Effects of Endogenous Treatments with Interference and Spillovers in a Large Network

This paper studies the identification and estimation of heterogeneous effects of an endogenous treatment under interference and spillovers in a large single-network setting. We model endogenous treatment selection as an equilibrium outcome that explicitly accounts for spillovers and derive conditions guaranteeing the existence and uniqueness of this equilibrium. We then identify heterogeneous marginal exposure effects (MEEs), which may vary with both the treatment status of neighboring nodes and unobserved heterogeneity. We develop estimation strategies and establish their large-sample properties. Equipped with these tools, we analyze the heterogeneous effects of import competition on U.S. local labor markets in the presence of interference and spillovers. We find negative MEEs, consistent with the existing literature. However, these effects are amplified by spillovers in the presence of treated neighbors and among localities that tend to select into lower levels of import competition. These additional empirical findings are novel and would not be credibly obtainable without the econometric framework proposed in this paper.

==> old_content_storage.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%% 250830 old treatment decision
\subsection{Game of Treatment Decisions}
Given the publicly observed network $A$, we assume that individuals make simultaneous treatment decisions in an incomplete information game. An individual $i$'s type is defined by a pair $(Z_i,\nu_i)$. Within a pair, $Z_i$ is commonly observed by all individuals but $\nu_i$ is private information that is only known to $i$. We write $\bfZ=(Z_1,...,Z_n)$, which is the public information observed by all individuals.

Given other individual's decisions $\bfD_{-i}$, an agent $i$ will obtain the payoff
\begin{equation} \label{equ:payoff}
    % u_i = \beta x_i+ \gamma z_i + \lambda \sum_j a_{ij} p_j - \nu_i
    u_i(Z_i,\bfD_{-i},\nu_i) = Z_i'\beta_D + \lambda  \sum_{j\neq i} a_{ij} D_j - \nu_{i}
\end{equation}
if she chooses to take the treatment ($D_i=1$) and 0 otherwise ($D_i=0$). In the payoff function, $\beta_D$ are the coefficients associated with $Z_i$ and $\lambda$ is the spillover effect on treatment take-up decision. Let $\bm{\beta}_1=(\beta_D',\lambda)'$. In the incomplete information game, the agent $i$ can only make a decision based on her belief in others' decisions. The  $i$'s strategy is then a mapping from her private information to treatment take-up decision conditional on public information:
% Let $\bfp=(p_1,...,p_n)$ be the agent $i$'s belief of the probabilities that other agents will take the treatment.
\begin{equation}\label{equ:BNEdesion}
\begin{aligned}
    D_i^*(\nu_i|\bfZ;\bm{\beta}_1)&=\mathbbm{1}\{E[u_i(Z_i,\bfD_{-i},\nu_i)|\bfZ,\nu_i]\geq 0\}\\
    &=\mathbbm{1}\{Z_i'\beta_D + \lambda \sum_{j\neq i} a_{ij} Pr\left(D_j^*(\nu_j|\bfZ;\bm{\beta}_1)=1| \bfZ,\nu_i \right)  \geq \nu_i \}
\end{aligned}
\end{equation}
Equation (\ref{equ:BNEdesion}) gives a system of equations that defines a BNE. We impose the following assumption

\begin{asm}\label{asm:iid} 
\begin{itemize}
    \item[]
    \item[(i)] Conditional on $\bfX$, the private information $\nu_i,i=1,..,n$ are $i.i.d$ random variable that follow logistic distribution.
    \item[(ii)] $\nu_i$ is conditionally independent of $\bfZ$ given $\bfX$.
\end{itemize}
\end{asm}

Assumption \ref{asm:iid}(i) is commonly imposed in the literature of incomplete information game \citep{Brock2:02,Bajari4:10,Xu:18}.
\red{find spatial literature}


With the assumption, $i$'s belief on other's choice probability is independent to its own private information $\nu_i$. Thus, we can write such belief as $\pi_i(\bfZ)=Pr(D_i^*(\nu_i|\bfZ;\bm{\beta}_1)=1|\bfZ)$. We also impose Assumption \ref{asm:iid}(ii) for identification of marginal treatment effects. Under Assumption \ref{asm:iid}, the beliefs $\Pi^*(\bfZ)=(\pi_1^*(\bfZ),...,\pi_n^*(\bfZ))$ should be self-consistent: they solve the following system of equations
\begin{equation}\label{equ:EQUcp}
\begin{aligned}
    \pi_1^*(\bfZ)&= F_{\nu|\bfX}(Z_1'\beta_D + \lambda \sum_j a_{1j} \pi_j^*(\bfZ)),\\
    &\vdots\\
    \pi_n^*(\bfZ)&= F_{\nu|\bfX}(Z_n'\beta_D + \lambda \sum_j a_{nj} \pi_j^*(\bfZ)),
\end{aligned}
\end{equation}
where $F_{\nu|\bfX}$ is the CDF of logistic distribution function given Assumption \ref{asm:iid}(i). 

% \red{Note: The conditioning is because $\bfZ$ enters the argument of $\nu$'s CDF. Moreover, since $\bfZ$ contains whole $\bfX$, the assumption will make conditoning only on $\bfX$. This is consistent with \cite{Heckman2:05,Hoshino2:23}}
\subsection{Conditions for Unique Equilibrium and Computation}
The existence of the solution for (\ref{equ:EQUcp}) follows from Brouwer's fixed-point theorem. We now characterize the conditions under which this solution is unique. Let $\parallel\cdot\parallel_1$ and $\parallel\cdot\parallel_\infty$ be the maximum row sum and column sum of a matrix.
\begin{asm}\label{asm:Small_spillover} \citep{Lee3:14} Let the absolute value of the spillover effect
\begin{equation}
    |\lambda| < \frac{1}{min(\parallel A\parallel_1,\parallel A\parallel_\infty)\cdot \underset{\nu}{max} f_{\nu|\bfX}(\nu)}.
\end{equation}
\end{asm}
\cite{Lee3:14} observed that when the selection peer effect $\lambda$ is small, the norm of the Jacobian matrix governing agents' belief updates will smaller than 1. Consequently, this ensures the existence of a unique equilibrium. We summarize the discussion in the following Lemma.
\begin{lemma}\label{lemma:UniBNE}
    Suppose Assumptions \ref{asm:iid} and \ref{asm:Small_spillover} hold. There will always be a unique solution for the system of equations (\ref{equ:EQUcp}).
\end{lemma}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 250827 old introduction
Endogenous treatment take-up is ubiquitous in the causal inference literature.%
\footnote{For example, \cite{Abadie:03,Frölich2:13,Donald3:14,Chernozhukov3:15,Kitagawa:15,Hsu3:22,Mogstad3:24}}
At the same time, understanding the treatment effect when observations are subject to interference has received increasing attention.%
\footnote{For example, \cite{Manski:93,Leung:15,Aronow2:17,Hu3:22,Cooprider2:23,DiTraglia4:23}}
This paper examines the intersection of these two challenges. Specifically, we discuss the identification and estimation of marginal treatment effect (MTE) with non-prefect compliance in a large single network setting.

Empirical studies are often motivated to learn the average treatment effects of policy or environmental changes, but resort to identifying the local average treatment effect due to endogeneity issues. As the two parameters are generally different, it is natural to investigate the extent of their difference. \cite{Björklund2:87} and other papers in the line of MTE literature provide a unified framework to study these two parameters. In the context of networks, there are studies that explore how we can learn the treatment effect with both the exogenous or endogenous treatment take-up\citep{Leung:22ECTA,Hoshino2:23_JSAS,Vazquez-Bare:23,Savje:23}. On the other hand, we still know relatively little about how to identify and estimate the MTE in the setting, the building block of the unified study framework.

Estimating the MTE requires (i) a structural model characterizing individual's treatment decision and (ii) how the treatment determines the outcomes. In a network, both the decisions and outcomes are likely to depend on others. For example, when assessing how import competition affects local labor market, one region's response can influence neighboring regions' labor market through labor's migration. Moreover, preferences for imported goods may spill over across regional borders. Thus, the model must accommodate interference in both treatment decisions and outcomes.

We begin by modeling the treatment choice. Following \cite{Xu:18}, we adopt an incomplete information game framework and derive the conditions under which a unique equilibrium exists. The uniqueness, in turn, allows us to point-identify the propensity score. Moving into the treatment effect stage, and following the literature of causal inference literature on network \citep{Leung:22ECTA,Hoshino2:23_JSAS}, we assume the existence of exposure mapping, a low-dimensional statistic that summarizes the interference in this network setting. Under this assumption, we show that the marginal response parameter can be identified without any additional functional form assumptions on the outcome model.

We estimate the model using the generalized method of moments (GMM). To analyze the statistical properties of the estimator, we adopt the conditional $\psi$-dependent framework developed by \cite{Kojevnikov3:21}, which characterizes the weak dependence between observations. Conditioning on the limiting $\sigma$-field generated by the common factors, we show that the estimator satisfies conditional consistency and stably converges to a mixture of normal distributions. Given the stable convergence, we can rescale the parameter with a proper variance estimator and implement the standard inference.

We illustrate the method with the \cite{Autor3:13} dataset on Chinese import competition and the manufacturing employment share across U.S. commuting zones(CZs). Treating each CZ as an independent open economy, their 2SLS documents a large negative effect of import competitions on manufacturing employment. However, as CZs are linked geographically, there might be interference on the degree of exposure in labor markets. We model the sector composition decisions as an incomplete information game on this spatial network. The result suggests that there is a strategic substitution in leaning toward sectors that face more competition from China. We further inspect the direct marginal effect of import competitions on the local labor market. We found that there is sizable difference between CZs with and without treated neighbors, the CZs that faces more import competition than the other half of CZs. These findings highlights the importance of considering network structure in evaluating treatment effect.

This paper is related to the studies of endogenous treatment where the interference is confined within each group or market. For example, \cite{Hoshino2:23} examine how the delinquency of the opposite gender best friend on student's GPA; \cite{Balat2:23} investigate how competition between airlines influences the air pollution in cities in the U.S. In both cases, they are able to identify the outcomes under all possible treatment patterns and make comparison accordingly. In contrast, this paper considers the setting where all individuals are connected by a large single network. As well documented in the network causal inference literature, it is impossible to identify all outcome parameters without any restriction of how outcomes vary with population treatment status. As a result, the existence of exposure mapping is often maintained in literature of network causal inference \citep{Leung:22ECTA,Hu3:22,Hoshino2:23}.

This paper is also broadly related to conditional inference frameworks for extreme estimators considered in \cite{Kuersteiner2:13} and \cite{Menzel:2015}. As our asymptotic results are all conditioning on the limiting $\sigma$-field with respect to which the network is measurable, it can be viewed as that our estimator enjoys the asymptotic properties shown in this paper regardless of the underlining network formation models provided that the sequences of networks are sufficiently sparse.

The rest of the paper is organized as follows. Section 2 presents the model setup. Section 3 establishes identification conditions for both stages. We propose an estimator in Section 4 proposes the estimator, and Section 5 analyzes its large sample properties. Finally, we numerically illustrate our estimator through simulation in Section 6.
